Logical Relations for Partial Features and Automatic Differentiation Correctness

We present a simple technique for semantic, open logical relations arguments about languages with recursive types, which, as we show, follows from a principled foundation in categorical semantics. We demonstrate how it can be used to give a very straightforward proof of correctness of practical forward- and reverse-mode dual numbers style automatic differentiation (AD) on ML-family languages. The key idea is to combine it with a suitable open logical relations technique for reasoning about differentiable partial functions (a suitable lifting of the partiality monad to logical relations), which we introduce.

==> SHORTassignment-functor-universalproperty-syntax.tex <==
\tiny\[
\begin{array}{c}
H(\reals) \in  \obb{\catV};\, H (\tSign)  \in   \ehomV{H(\reals)} {T\left( \terminall\sqcup \terminall\right)}; 
H (\cnst c) \in   \ehomV{\terminall}{H(\reals)}; \, 
H (\op)\in   \ehomV{H(\reals)^n }{ TH(\reals) }.
\end{array}
\] 
\normalsize 
 


==> SHORTassignment-universalproperty-syntax-target.tex <==
\tiny
\[
\begin{array}{c}
	\extendedH{H}( \tangentreals ) \in   \obb{\catV}; \, \extendedH{H} (\cnzero ) \in   \ehomV{\terminall}{\extendedH{H} (\tangentreals )}; \,\extendedH{H}\left( \tangentprojection{i}{}\right) \in \ehomV{\tangentreals }{\targetreals ^i }    \mbox{ (for each  $i\in\NN ^\ast$)} ;
\\ 
	\extendedH{H} (+)\in   \ehomV{\extendedH{H}(\tangentreals )^2 }{ T\extendedH{H} (\tangentreals ) }; \,
\extendedH{H} (\ast )\in   \ehomV{\extendedH{H}(\tangentreals )\times \extendedH{H}  \left(\reals \right) }{ T\extendedH{H} \left( \tangentreals \right) }.
\end{array}
\] 
\normalsize  
			



==> app-macro.tex <==
\begin{figure}[!ht]
	\fbox{\parbox{0.98\linewidth}{\begin{minipage}{\linewidth}\noindent
				\input{d-types1SHORT}
				\hrulefill
				\input{d-terms1SHORT}
	\end{minipage}}}
	\caption{AD macro  $\Dsyn{-}$ defined on types and computations.
		All newly introduced variables are chosen to be fresh.}
		%	We single out the rule for constants $\cnst{c}$, primitive operations $\op$ and $\tSign$, as %   this is where the interesting work specific to differentiation happens.
		%We provide a more efficient way of differentiating $\tSign$ in Appx. \ref{sec:efficient-sign-derivative}. \label{fig:ad1}}
\end{figure}

==> d-terms2SHORT.tex <==
\[
    \begin{array}{ll}
    \Dsynplain{\tRoll{\trm{1}}} \defeq \tRoll{\Dsyn{\trm{1}}}\qquad &\Dsynplain{\rMatch{\trm{1}}{\var{1}}{\trm{2}}}\defeq 
    \rMatch{\Dsynplain{\trm{1}}}{\var{1}}{\Dsynplain{\trm{2}}} 
    \end{array}
    \]

==> d-types-terms3SHORT.tex <==
\[
    \begin{array}{lll}
        \Dsynplain{\forall\tvar{1}.\tysch{1}} \defeq {\forall.\tvar{1}}.\Dsynplain{\tysch{1}}   \qquad
         & \Dsynplain{\Lambda\tvar{1}.\trm{1}}\defeq\Lambda\tvar{1}.\Dsynplain{\trm{1}}\qquad &\Dsynplain{\trm{1}\,\ty{1}}\defeq 
    \Dsynplain{\trm{1}}\,\Dsynplain{\ty{1}}
\end{array} 
    \]

==> d-types2SHORT.tex <==
\[
\begin{array}{lll}
\Dsynplain{\tvar{1}} \defeq {\tvar{1}}\qquad & \Dsynplain{\trec{\tvar{1}}{\ty{1}}} \defeq \trec{\tvar{1}}{\Dsynplain{\ty{1}}}
& \end{array}    
\]

